Can Vision-Language Models Count? A Synthetic Benchmark and Analysis of Attention-Based Interventions

Recent research suggests that Vision Language Models (VLMs) often rely on inherent biases learned during training when responding to queries about visual properties of images. These biases are exacerbated when VLMs are asked highly specific questions that require selective visual attention, a demand that mirrors cognitive challenges observed in human enumeration tasks. We build upon this research by developing a synthetic benchmark dataset and evaluation framework to systematically characterize how counting performance varies as image and prompt properties change. Using open-source VLMs, we analyze how performance shifts across controlled perturbations (e.g. number of objects, object color, background color, object texture, background texture, and prompt specificity) and examine corresponding changes in visual attention allocation. We further conduct exploratory attention reweighting experiments in the language model decoder to modulate focus on visual tokens at different layers and assess their effects on counting behavior. Our results reveal that counting accuracy degrades systematically with increasing visual and linguistic complexity echoing human limits and cognitive load effects known from human perception, while targeted attention reweighting yields modest but measurable improvements. Rather than competing on benchmark accuracy, we introduce a controlled diagnostic framework for analyzing VLM enumeration behavior. Through systematic experiments, we expose failure modes rooted in cross-modal binding that natural image benchmarks may not easily isolate, and provide preliminary empirical evidence that targeted attention reweighting in the language decoder can influence how models ground linguistic quantity concepts in visual representations. Code and data available here: https://github.com/ssen7/vlm-count-analysis

==> sec/6_Limitations.tex <==
\section{Limitations}
\label{sec:limitations}
While our controlled synthetic benchmarks enable precise failure mode analysis, extending this framework to real-world scenarios with occlusion, varying scales, and complex spatial arrangements remains essential. 
Our attention interventions assume standard transformer architectures; if frontier models employ attention variants (e.g., mixture of depths or sparse attention patterns), our strategies may not directly transfer.
% Our attention intervention experiments are conducted exclusively on the background texture subset, and it remains unclear whether the observed trends generalize across other visual conditions in our benchmark. 
Finally, our analysis is limited to open-source VLMs; proprietary and larger-scale models may exhibit qualitatively different failure modes and responses to attention intervention.
% While our controlled synthetic benchmarks enable precise failure mode analysis, extending this framework to real-world scenarios with occlusion, varying scales, and complex spatial arrangements remains essential. 
% Creating "naturalistic" synthetic datasets that interpolate between our controlled stimuli and real images could help identify which visual complexity factors transfer to practical counting applications.
% Our evaluation framework did not incorporate reasoning-augmented versions of the tested models, such as Kimi-VL-A3B-Thinking \cite{kimiteam2025kimivltechnicalreport}, which employ extended chain-of-thought (CoT) reasoning. Our evaluation exclusively examines open-source VLMs—while methodologically necessary for attention introspection—limits our assessment of the broader landscape of VLM counting capabilities. Proprietary models may also employ inference-time techniques we cannot observe or replicate. Furthermore, our attention interventions assume standard transformer architectures; if frontier models employ attention variants (e.g., mixture of depths or sparse attention patterns), our strategies may not directly transfer. Finally, while synthetic data enables controlled variable manipulation, it may not fully capture the visual complexity of natural images, potentially limiting the generalizability of our findings. 

% While our controlled synthetic benchmarks enable precise failure mode analysis, extending this framework to real-world scenarios with occlusion, varying scales, and complex spatial arrangements remains essential. Creating "naturalistic" synthetic datasets that interpolate between our controlled stimuli and real images could help identify which visual complexity factors transfer to practical counting applications.
% Our evaluation framework did not incorporate reasoning-augmented versions of the tested models, such as Kimi-VL-A3B-Thinking or QwQ-32B-Preview, which employ extended chain-of-thought (CoT) reasoning through reinforcement learning and long-horizon thinking mechanisms. This represents a significant gap in our analysis for several reasons.Our exclusive reliance on synthetic benchmarks, while methodologically advantageous for controlled variable manipulation, introduces limitations that could constrain the generalizability of our findings.  Our evaluation exclusively examines open-source VLMs—Qwen2.5-VL, Kimi-VL-A3B, and InternVL3-9B—which, while methodologically necessary for attention introspection, introduces significant limitations in assessing the broader landscape of VLM counting capabilities and the generalizability of our proposed interventions. Proprietary models may also employ inference-time techniques we cannot observe or replicate. Our attention interventions operate at the architectural level, assuming standard transformer attention mechanisms; if frontier models employ attention variants (e.g., mixture of depths, sparse attention patterns, or dynamic routing mechanisms), our intervention strategies may not transfer.

% \begin{itemize}
%     \item Did not use reasoning versions of the models.
%     \item confined to synthetic data.
%     \item only evaluated on open source models.
% \end{itemize}

==> table_compact.tex <==
\begin{table}[htbp]
\centering
\caption{Model Performance Comparison on FSC-147. \textbf{Bold} methods beat baseline for both models in MRCE.}
\label{tab:rwd_model_comparison}
\footnotesize % Even smaller font for compact display
\setlength{\tabcolsep}{3pt} % Reduce column spacing
\begin{tabular}{@{}lrrr|rrr@{}}
\toprule
& \multicolumn{3}{c}{\textbf{Qwen3VL-8B (Dense)}} & \multicolumn{3}{c}{\textbf{Kimi (MoE)}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method} & \textbf{Acc.} & \textbf{V.} & \textbf{MRCE} & \textbf{Acc.} & \textbf{V.} & \textbf{MRCE} \\
\midrule
Early Amp. VM & .224 & 49 & .143 & 18.4 & 49 & .344 \\
Late Vis. Ret. & .224 & 49 & .145 & 24.0 & 50 & .725 \\
Uniform Bal. & .163 & 49 & .158 & 22.0 & 50 & .694 \\
Early Amp. VM BG & .200 & 50 & .160 & 18.4 & 49 & .344 \\
Prog. Vis. Grow & .240 & 50 & .163 & 26.0 & 50 & .694 \\
\textbf{Late Amp. VM} & \textbf{.204} & \textbf{49} & \textbf{.163} & \textbf{14.3} & \textbf{49} & \textbf{.296} \\
\textbf{Extreme Text} & \textbf{.160} & \textbf{50} & \textbf{.164} & \textbf{22.0} & \textbf{50} & \textbf{.297} \\
Baseline & .220 & 50 & .168 & 16.0 & 50 & .301 \\
Late Amp. VM BG & .260 & 50 & .172 & 14.3 & 49 & .296 \\
Alt. Amp Sup & .220 & 50 & .176 & 16.0 & 50 & .332 \\
Mid. Vis. Boost & .208 & 48 & .185 & 28.0 & 50 & .307 \\
Uniform Amp. & .234 & 47 & .192 & 20.0 & 50 & .347 \\
Mid. Amp. VM & .224 & 49 & .195 & 16.3 & 49 & .281 \\
Prog. Vis. Fade & .163 & 49 & .218 & 20.0 & 50 & .738 \\
Mid. Amp. VM BG & .120 & 50 & .225 & 16.3 & 49 & .281 \\
Uniform Sup. & .120 & 50 & .226 & 14.0 & 50 & .326 \\
Uniform Focus & .000 & 0 & --- & 20.0 & 50 & .374 \\
Early Vis. Only & .000 & 0 & --- & 18.0 & 50 & .429 \\
Extreme Vis. Early & .000 & 0 & --- & 16.0 & 50 & .771 \\
\bottomrule
\end{tabular}
% \begin{tablenotes}
% \footnotesize
% \item Acc. = Accuracy (\%), V. = Valid Predictions, MRCE = Mean Relative Count Error
% \item \textbf{Bold methods:} Beat baseline (MRCE: Qwen < 0.168, Kimi < 0.301) for both models
% \item Amp. = Amplify, Vis. = Visual, VM = Visual Mask, BG = Background Suppress
% \item Prog. = Progressive, Ret. = Retention, Bal. = Balance, Sup. = Suppress, Alt. = Alternating, Mid. = Middle
% \end{tablenotes}
\end{table}

